Optimizing Quantum Programs against Decoherence: Delaying Qubits into Quantum Superposition

Quantum computing technology has reached a second renaissance in the last decade. However, in the NISQ era pointed out by John Preskill in 2018, quantum noise and decoherence, which affect the accuracy and execution effect of quantum programs, cannot be ignored and corrected by the near future NISQ computers. In order to let users more easily write quantum programs, the compiler and runtime system should consider underlying quantum hardware features such as decoherence. To address the challenges posed by decoherence, in this paper, we propose and prototype QLifeReducer to minimize the qubit lifetime in the input OpenQASM program by delaying qubits into quantum superposition. QLifeReducer includes three core modules, i.e.,the parser, parallelism analyzer and transformer. It introduces the layered bundle format to express the quantum program, where a set of parallelizable quantum operations is packaged into a bundle. We evaluate quantum programs before and after transformed by QLifeReducer on both real IBM Q 5 Tenerife and the self-developed simulator. The experimental results show that QLifeReducer reduces the error rate of a quantum program when executed on IBMQ 5 Tenerife by 11%; and can reduce the longest qubit lifetime as well as average qubit lifetime by more than 20% on most quantum workloads.

==> backups.tex <==
By rewriting the code, changing it to a bundle format we can clearly identified a $PGSO$ instruction. In Fig.\ref{main_example}, We can find that qubit q[0] enter superposition state in line-3. It is used in line-4 and line-7. In fact, we can move those two instruction about q[0] in line-3 and line-4 downto line-5 and line-6. Then the program will become Fig.\ref{main_example_done}
\begin{figure}[h]
\centering
\begin{lstlisting}
qreg q[5];
creg c[3];
h q[1]; h q[2]; 
s q[1]; s q[2]; 
cx q[1],q[2]; h q[0];
tdg q[2]; s q[0];
cx q[0],q[2];
t q[2];
\end{lstlisting}
\caption{Part of Grover algorithm in bundle format after transformation}
\label{main_example_done}
\end{figure}
This transformation will not change the program's origin effect while reduce the time q[0] remain in superposition thus the error rate will decrease.


 \begin{figure*}[htbp]
\centering
\subfigure[]{
  \label{fig::tranbeforecode}
  \includegraphics[width=0.18\textwidth]{figs/before/tranbeforecode.png}
}
\subfigure[]{
  \label{fig::tranbeforegraph}
  \includegraphics[width=0.30\textwidth]{figs/before/tranbefore.png}
}
\subfigure[]{
  \label{fig::tranaftercode}
  \includegraphics[width=0.18\textwidth]{figs/after/tranaftercode.png}
}
\subfigure[]{
  \label{fig::tranaftergraph}
  \includegraphics[width=0.30\textwidth]{figs/after/tranafter.png}
}

\caption{Quantum circuit before and after translation and its bundle format in topological structure}
\label{sec:transformation}
\end{figure*}

==> code.tex <==
源代码：
原本版本：
qreg q[16];
h q[1];
h q[2];
cx q[2], q[3];
h q[2];
h q[6];
cx q[6], q[11];
cx q[1], q[2];
h q[11];
h q[6];
cx q[6], q[11];
cx q[11], q[1];

原本情况下的分层：
0: h q[1]; h q[2]; 
1: cx q[2], q[3]; 
2: h q[2]; h q[6]; 
3: cx q[6], q[11]; cx q[1], q[2]; 
4: h q[11]; h q[6]; 
5: cx q[6], q[11]; 
6: cx q[11], q[1]; 
*---------------------
共7层

经过变换后：
0: h q[2]; h q[6]; 
1: cx q[2], q[3]; cx q[6], q[11]; 
2: h q[1]; h q[2]; h q[11]; h q[6]; 
3: cx q[1], q[2]; cx q[6], q[11]; 
4: cx q[11], q[1]; 
*---------------------
仅有5层，展开后即是变换后的代码
h q[2];
h q[6];
cx q[2], q[3];
cx q[6], q[11];
h q[1];
h q[2];
h q[11];
h q[6];
cx q[1], q[2];
cx q[6], q[11];
cx q[11], q[1];

与普通压缩的不同之处是还推迟了q[1]进入叠加态的时间，将h q[1]操作从第一层推迟到了第二层。



==> discuss.tex <==
将之前的实验数据汇总，描述进行评测的代码和平台的参数，评测的正确率和错误率的依据。IBM目前支持的量子门：
单量子门：X,Y,Z,H,S,T,Steg,Tteg,UI
双量子门只有CNOT
测试样例使用的门：H,X,T,CNOT以及测量操作


程序测试集:
    在论文文件夹下，存有两个代码文件夹(命名直白)均有说明文档。
    至于支持的测试代码，现在暂未测试。但可以肯定的是，很大一部分并不被目前测试程序支持。但问题不大，因为原因跟算法本身无关，主要是openqasm自身实现的一些编程功能，如函数调用，判断语句
    
cirq related Link:  
    
    
    知乎专栏转载:     https://juejin.im/entry/5c23dc29f265da61570587c7
    
    github地址:
    https://github.com/quantumlib/Cirq
    
    在optimizer.py \_accept函数中采用模拟时间指数衰减函数(主要为状态概率估计)
    
    进一步信息，仍需时间进行考虑。
    
    测试程序的共同特征：变换前后代码中，对于q[1]的H门操作都在一开始。变换前代码，对于q[0]和q[1]之间的CNOT操作中间隔了一段时间，一般含有一次对其他不相关比特的测量。而变换后代码中，q[0]和q[1]之间的CNOT操作始终紧跟在对于q[1]的H门操作后


评估方法：
    1.门的总数
    Number of one-qubit gates and CNOT (or any other two-qubit gate) is a complexity metric for quantum synthesis algorithms. Since CNOT is a linear gate, the number of one-qubit gates (excluding inverters) needed to express a computation is defined as a measure of non-linearity for a given computation [Shende and Markov 2009].
    \cite{saeedi2013synthesis}
    原文：On the CNOT-cost of TOFFOLI gates
    2.层的总数（邓皓巍：算法不会增加层数，证明？）
        Depth (or the number of levels) is defined as the largest number of elementary gates on any path from inputs to outputs in a circuit. When any subset of gates can be invoked simultaneously, decreasing circuit depth reduces circuit latency. This assumption is trivial for conventional semiconductor circuits because the gates are manufactured individually and exist at the same time. However, when quantum gates are invoked by electromagnetic pulses, their parallel invocation must clear a number of obstacles — it should be possible to select just the right set of qubits on which the gates are applied, which may require several laser sources and possibly several pre-determined wavelengths. When the parallel gates perform different functions, interference between them may limit achievable parallelism. Practical quantum computers can either apply the same gate to all qubits or apply different gates to a small number of qubits.
        \cite{saeedi2013synthesis}
        2.1.层数的加权和（主要是，CX等门实现的要慢一些Operations supported by this quantum process or include measurements, single-qubit x- or y-axis rotations, and a two-qubit controlled-phase(CZ)gate.  typical gate time is 20ns for single qubit gates and ∼ 40 ns for two-qubit gates. The duration of a measurement is typically 300ns-1µs. A cycle time of 20 ns is used in this instantiation.
        \cite{fu2018eQASM}）
    3.量子比特处于非基态的时间（下称为生存时间）。
      从第一个门作用到该比特开始，到测量操作
      （或者对于辅助比特是最后一）门操作，
      这里假设已进行结尾无用代码删除）为止。
      这个指标主要是对消相干的考虑。
      设每个量子比特的生存时间为$T_i$：
        3.1.平均生存期$\frac{\sum_i T_i}{n}$
        3.2.最长生存期$max\{ T_i \}$，
            最长生存期对程序错误往往有比较重要的意义，
            因为这个比特最容易出错。
        3.3.消相干水平（这个称谓可能不准确，修改？）
            $D_i=e^{-\frac{T_i}{\tau} }$，这里$\tau$是T1或T2。
            对应的，可以有平均消相干水平来衡量整个电路的消相干问题。



OpenQasm画图工具 qasm2cirq

readme ::
REQUIREMENTS:
- latex2e with xypic (included in tetex)
- python version 2.3 or greater
- ghostscript (and epstopdf)
- netpbm (for creation of png files)
-----------------------------------------------------------------------------
USAGE:
qasm2pdf <qasmfile>
qasm2png <qasmfile>

Example: qasm2pdf test2.qasm

用来将qasm代码生成对应电路图，较为方便观看测试程序图形

测试程序来源:

QasmProgrm 
generated by ProjectQ.IBMBackend
https://github.com/ProjectQ-Framework/ProjectQ/tree/develop/examples

Quantum-Computing-master:
https://github.com/sampaio96/Quantum-Computing

qiskit\_openqasm\_example:
https://github.com/Qiskit/openqasm/tree/master/examples



How to use Tikz to show gate-pic?

Firstly, using  qpic to program quantum circuit is convenient.
But for simple gates , I recommend modifing Tikz code indirectly .
for example ,
if you want to insert the pic generated by tikz into pdf ,you can use 
the following two commands in .tex .

% \usepackage{tikz}
% \input{filename.tikz}

if you will use X gate ,just use X.tikz. And  'filename.tikz' refers to 'X.tikz' now. 

another-way but no need.
link :  https://stackoverflow.com/questions/3248816/latex-tikz-and-separate-compilation-of-chapters-and-figures

paper cgo2018中，随机生成测试程序
 To complement this set of microbenchmarks, we have
also generated synthetic QASM programs. These programs
are randomly generated quantum circuits with uniformly
distributed dependences.

scaffcc中认为指令按照尽快执行的方式执行
Adhering to these dependencies, the critical
path timing analysis schedules operations by reordering instructions
in as-soon-as-possible (ASAP) order.

==> ex-qasm2.tex <==
\begin{figure}[htbp]
\centering
%\footnotesize
\scriptsize
\begin{minipage}[c]{.17\textwidth}
\centering
\begin{lstlisting}
qreg q[5];
creg c[3];
<@\textcolor{blue}{h q[0]; h q[1]; h q[2];}@>
<@\textcolor{blue}{s q[0]; s q[1]; s q[2];}@>
cx q[1],q[2];
tdg q[2];
cx q[0],q[2];
t q[2];
\end{lstlisting}
{(a) Before}
\label{fig:ex:qasm:a}
%\subcaption{(a) Before}
\end{minipage}
\hfill
\begin{minipage}[c]{.1\textwidth}
\centering
\includegraphics[width=0.95\textwidth]{figs/ex-qasm2.jpg}
\qquad
\\
{(b) Layered \\dependence graph}
%\subcaption{(b) After}
\label{fig:ex:qasm:b}
\end{minipage}
\begin{minipage}[c]{.21\textwidth}
\centering
\begin{lstlisting}
qreg q[5];
creg c[3];
h q[1]; h q[2];
s q[1]; s q[2];
cx q[1],q[2]; <@\textcolor{blue}{h q[0];}@> 
tdg q[2]; <@\textcolor{blue}{s q[0];}@>
cx q[0],q[2];
t q[2];
\end{lstlisting}
{(c) After}
\label{fig:ex:qasm:c}
%\subcaption{(a) Before}
\end{minipage}
%}
%}
\caption{OpenQASM program example: ackage operations into layers}
\label{fig:ex:qasm2}
\end{figure}



==> gates.tex <==
Quantum logic gate
 Hadamard (H) gate
$$\LARGE{
	H=\frac{1}{\sqrt 2}
	\begin{bmatrix}
	1 & 1	\\
	1 & -1
	\end{bmatrix}
}
$$



Pauli\-X gate
$$\LARGE{
	X=
	\begin{bmatrix}
	0 & 1	\\
	1 & 0
	\end{bmatrix}
}​$$
等价于经典计算机中的非门（NOT)
 Pauli-Y gate
$$\LARGE{
	Y=
	\begin{bmatrix}
	0 & -i	\\
	i & 0
	\end{bmatrix}
}​$$
 Pauli-Z gate
$$\LARGE{
	Z=
	\begin{bmatrix}
	1 & 0	\\
	0 & -1
	\end{bmatrix}
}​$$
有时被称作相位翻转（phase-filp) 
$X^2=Y^2=Z^2=I​$
 Square root of NOT gate
$$\LARGE{
	\sqrt{X}=\sqrt{NOT}=\frac{1}{2}
	\begin{bmatrix}
	1+i & 1-i	\\
	1-i & 1+i
	\end{bmatrix}
}​$$
 Phase shift gates
$$\LARGE{
	R_{\phi }=
	\begin{bmatrix}
	1 & 0	\\
	0 & e^{i\phi}
	\end{bmatrix}
}​$$
 Swap gate
$$\LARGE{
	SWAP=
	\begin{bmatrix}
	1 & 0 & 0 & 0	\\
	0 & 0 & 1 & 0	\\
	0 & 1 & 0 & 0	\\
	0 & 0 & 0 & 1
	\end{bmatrix}
}​$$
 Square root of Swap gate
$$\LARGE{
	\sqrt{SWAP}=
	\begin{bmatrix}
	1 & 0 & 0 & 0	\\
	0 & \frac{1}{2}(1+i) & \frac{1}{2}(1-i) & 0	\\
	0 & \frac{1}{2}(1-i) & \frac{1}{2}(1+i) & 0	\\
	0 & 0 & 0 & 1
	\end{bmatrix}
}​$$
$\sqrt{SWAP}​$是通用的，任何多量子门都能由$\sqrt{SWAP}​$和单量子门构成\
 Control gates
$$\LARGE{
	C(U)=
	\begin{bmatrix}
	1 & 0 & 0 & 0	\\
	0 & 1 & 0 & 0	\\
	0 & 1 & u\_{00} & u\_{01}	\\
	0 & 0 & u\_{10} & u\_{10}
	\end{bmatrix}
}​$$
 Toffoli gates
$$\LARGE{
	CCNOT=
	\begin{bmatrix}
	1 & 0 & 0 & 0 & 0 & 0 & 0 & 0	\\
	0 & 1 & 0 & 0 & 0 & 0 & 0 & 0	\\
	0 & 0 & 1 & 0 & 0 & 0 & 0 & 0	\\
	0 & 0 & 0 & 1 & 0 & 0 & 0 & 0	\\
	0 & 0 & 0 & 0 & 1 & 0 & 0 & 0	\\
	0 & 0 & 0 & 0 & 0 & 1 & 0 & 0	\\
	0 & 0 & 0 & 0 & 0 & 0 & 0 & 1	\\
	0 & 0 & 0 & 0 & 0 & 0 & 1 & 0	\\
	\end{bmatrix}
}​$$

CNOT
$$\LARGE{
	U_{CN}=
	\begin{bmatrix}
	1 & 0 & 0 & 0 	\\
	0 & 1 & 0 & 0 	\\
	0 & 0 & 0 & 1 	\\
	0 & 0 & 1 & 0 	\\
	\end{bmatrix}
}$$



Phase
$$\LARGE{
	S=
	\begin{bmatrix}
	1 & 0  	\\
	0 & i  	\\
	\end{bmatrix}
}​$$



$\pi$/8  
$$\LARGE{
	\pi/8 =
	\begin{bmatrix}
	1 & 0  	\\
	0 & e^{i\pi/4}  	\\
	\end{bmatrix}
}$$

==> measure.tex <==
\cite{fu2018QuMA}
It
is possible to make use of conventional processor design methods to optimize the nondeterministic
timing domain without affecting the deterministic timing of the output. Inspired by
conventional processor design techniques, such as the Intel Streaming SIMD Extensions (SSE),
we proposed a Single-Operation-Multiple-Qubit (SOMQ) execution fashion for QuMA in our
recent research. Together with a very-long-instruction-word architecture (VLIW) update, we
implemented the digital part of the improved QuMA in a device capable of controlling seven
qubits. With a slight change to the configuration, such as VLIW width, the device can be, in
principle, extended to control at least 49 qubits, which can form a distance-5 surface code logical
qubit.10

\cite{fu2019eQASM} 3.3 SOMQ
3.4 Very Long Instruction Word
Quantum Bundle Format
antum Bundle Format. Apart from SOMQ, dierent operations
are also allowed to be applied on dierent qubits in parallel.
eQASM can combine parallel quantum operations into a quantum
bundle in a VLIW format. We dene parallel quantum operations
as operations starting at the same timing point, regardless of the
duration of each operation. e format of a quantum bundle is:
[PI,] <Quantum Operation> [| <Quantum Operation>]*
e vertical bar | is used to separate dierent quantum operations
in the same bundle. e asterisk * means the item in square brackets
can repeat for n  0 times.

4.1 Target Superconducting antum Chip
A typical gate time is 20 ns for singlequbit
gates and  40 ns for two-qubit gates. e duration of a
measurement is typically 300 ns - 1 μs. A cycle time of 20 ns is used
in this instantiation.


==> related.tex <==
\section{Related Work}
\label{sec:rel}
\cite{steiger2018projectq}
ProjectQ is an open source compiler framework that allows optimization of cancelling one operation with its inverse including QFT,rotation gates and basic gates implemented, and merging rotation by default.For certain subroutines such as the multi-controlled NOT construction or the constant-addition circuit,it can optimize the allocation of such ancilla qubits by simply providing an unused qubit . We generate a few entangling quantum programs  based on it  and realize the qubit number used in specific procedures will be affected by some issues , such as the structure of the IBM chip.We find ProjectQ provides the integrated QFT gate in generated OpenQASM code , unlike ScaffCC that provides its concrete implementation. ~\cite{haner2018compiling}

\cite{abhari2014scaffcc}
ScaffCC is a scalable compiler for large-scale quantum applications, and show the opportunities for reducing compilation and analysis time, as well as output code size. %It is implemented in LLVM, a rich,  open-source library of compiler technologies, by adding intrinsic functions representative of quantum gates and a datatype representative of qubits.  With the applicability of some classical techniques and also opportunities for exploiting the dual classical-quantum nature of programs for keeping the compilation process tractable, ScaffCC is able to compile large-scale applications.Methods for program correctness checking as well as a novel approach to reversible-logic synthesis were applied, and the trade-off between optimality and speed in circuit timing analysis was also discussed while designing. 
In this paper, we evaluate the effect of QLifeReducer in the flat-format which is actually supported by the IBM, while ScaffCC prefers to analyze code in hierarchical-format. Also, we modified the cost of circuit by assigning different cost to different gates to conform better with reality. However, as a whole, we still follow the basic principle of parallelism and evaluation that showed in the ScaffCC.



\cite{fu2019eQASM}
eQASM is an executable quantum instruction set architecture based on QASM  that can be generated by the compiler backend from a higher-level representation, like OpenQASM\cite{cross2017OpenQASM} or cQASM.~\cite{fu2019eQASM} eQASM uses SOMQ execution, which can apply a single quantum operation on multiple qubits at the same time, and Very Long Instruction Word(VLIW)  which allows a instruction to express multiple operations to qubits at a single time. This paper considers the parallelism of quantum program in the same way as eQASM considered.



